DynamicFilter: an Online Dynamic Objects Removal Framework for Highly Dynamic Environments

Emergence of massive dynamic objects will diversify spatial structures when robots navigate in urban environments. Therefore, the online removal of dynamic objects is critical. In this paper, we introduce a novel online removal framework for highly dynamic urban environments. The framework consists of the scan-to-map front-end and the map-to-map back-end modules. Both the front- and back-ends deeply integrate the visibility-based approach and map-based approach. The experiments validate the framework in highly dynamic simulation scenarios and real-world datasets.

==> problem.tex <==
\section{Problem Formulation}
\label{sec:problem}

In this paper, we focus on the dynamic points removal from the consecutive 3D LiDAR scans. The point cloud $_B\mathcal{P}$ of each scan locates at the local sensor frame $B$. By advance LiDAR SLAM system\cite{shan2020lio,xu2021fast}, we can compute the transition $^B_W\mathbf{T}$ between local sensor frame $B$ and the global coordinate $W$. Thus, we associate the point cloud and its transition as a frame $_B\mathcal{F}$.






